Efficient Secure Aggregation for Privacy-Preserving Federated Machine Learning

Secure aggregation protocols ensure the privacy of users' data in federated learning by preventing the disclosure of local gradients. Many existing protocols impose significant communication and computational burdens on participants and may not efficiently handle the large update vectors typical of machine learning models. Correspondingly, we present e-SeaFL, an efficient verifiable secure aggregation protocol taking only one communication round during the aggregation phase. e-SeaFL allows the aggregation server to generate proof of honest aggregation to participants via authenticated homomorphic vector commitments. Our core idea is the use of assisting nodes to help the aggregation server, under similar trust assumptions existing works place upon the participating users. Our experiments show that the user enjoys an order of magnitude efficiency improvement over the state-of-the-art (IEEE S\&P 2023) for large gradient vectors with thousands of parameters. Our open-source implementation is available at https://github.com/vt-asaplab/e-SeaFL.

==> figs/exp/total_agg/agg_bandwidth.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{A}{HTML}{e6194B}%
\definecolor{B}{HTML}{f58231}%
\definecolor{C}{HTML}{4363d8}%
\definecolor{D}{HTML}{911eb4}%
\definecolor{E}{HTML}{3cb44b}%
\definecolor{F}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{G}{HTML}{808000}%
\definecolor{H}{HTML}{000000}%
%
\begin{tikzpicture}
\small	
	\begin{axis}[%
		width=0.8\textwidth,
		height=0.95\textwidth,
		at={(1.128in,0.894in)},
		scale only axis,
		xmin=0,
		xmax=6,
		xlabel={Number of users},
		xtick={0, 1, 2, 3, 4, 5, 6},
		xticklabels={$ $, $200$, $ 400 $, $ 600 $, $ 800 $, $ 1000 $},
		ymax=1000000000000000000,
            ymode=log,
            %ymax=100000,
            %ymode=log,
        %    ytick distance= 10,
		%ytick={0.01, 0.02, 0.02, 0.03, 0.04, 0.05, 0.06},
		ylabel = {Bandwidth (B)},
		ylabel shift=-5pt,
		yticklabel shift={0cm},
		axis background/.style={fill=white},
		legend columns=1,
		legend style={legend cell align=left, align=left, fill=none, draw=none,inner sep=-0pt, row sep=0pt, font=\scriptsize},
		legend pos = north west,
		%
		%ymajorgrids,
		%xmajorgrids,
		%grid style={line width=.1pt, draw=gray!90,dashed},
		%major grid style={line width=.1pt,draw=gray!50},
		minor y tick num=5,
		%legend style={at={(.97,0.76)}},
		]
		% \addplot [color=A, solid, mark=diamond*, mark options={solid, A}]
		% table[row sep=crcr]{%
		% 	1 11.0790\\ % 11.0790 ms
		% 	2 21.0162\\  %21.0162 ms
		% 	3 30.7832\\ 
		% 	4 40.9725\\ 
		% 	5 50.7883\\
		% };
		% \addlegendentry{E-seaML}

        \addplot [color=E, solid, mark=asterisk, mark options={solid, E}]
		table[row sep=crcr]{%
                1  13056040\\ 
			2  25856040\\ 
			3  38656040\\ 
			4  51456040\\ 
			5  64256040\\ 
		};
		\addlegendentry{\nano~(SH)}

  
		\addplot [color=A, solid, mark=diamond*, mark options={solid, A}]
		table[row sep=crcr]{%
			1 13056552\\ % 
			2 25856552\\ % 
			3 38656552\\ % 
			4 51456552\\ % 
			5 64256552\\ %
		};
		\addlegendentry{\nano~(MS)}
		
		\addplot [color=B, dashed, mark=square*, mark options={solid, B}]
		table[row sep=crcr]{%
			1 32838370883.2\\ % 
			2 98479396524.8\\ % 
			3 229761447806.4\\ % 
			4 410274268320\\ % 
			5 640017858064\\ % 
		};
		\addlegendentry{MicroFedML$_1$}

		\addplot [color=C, loosely dotted, mark=triangle*, mark options={solid, C}]
		table[row sep=crcr]{%
			1 32838370883.2\\ % 
			2 98479396524.8\\ % 
			3 229761447806.4\\ % 
			4 410274268320\\ % 
			5 640017858064\\ % 
		};
		\addlegendentry{MicroFedML$_2$(50)}


		\addplot [color=H, dashed, mark=pentagon*, mark options={solid, H}]
		table[row sep=crcr]{%
			1 40229664\\ % 
			2 80064448\\ %
			3 119898848\\ %
			4 159733632\\ %
			5 199568032\\ % 
		};
		\addlegendentry{\FlamingoServerFirst}

		\addplot [color=D, loosely dotted, mark=otimes*, mark options={solid, D}]
		table[row sep=crcr]{%
			1 120480544\\ %
			2 239777728\\ %
			3 359074528\\ %
			4 478371712\\ %
			5 597668512\\ % 
		};
		\addlegendentry{\FlamingoServerSec}


	\end{axis}


\end{tikzpicture}%


==> figs/exp/total_setup/setup_bandwidth.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{A}{HTML}{e6194B}%
\definecolor{B}{HTML}{f58231}%
\definecolor{C}{HTML}{4363d8}%
\definecolor{D}{HTML}{911eb4}%
\definecolor{E}{HTML}{3cb44b}%
\definecolor{F}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{G}{HTML}{808000}%
\definecolor{H}{HTML}{000000}%
%
\begin{tikzpicture}
\small	
	\begin{axis}[%
		width=0.8\textwidth,
		height=0.95\textwidth,
		at={(1.128in,0.894in)},
		scale only axis,
		xmin=0,
		xmax=6,
		xlabel={Number of users},
		xtick={0, 1, 2, 3, 4, 5, 6},
		xticklabels={$ $, $200$, $ 400 $, $ 600 $, $ 800 $, $ 1000 $},
		ymax=1000000000000000,
            ymode=log,
            %ymax=100000,
            %ymode=log,
        %    ytick distance= 10,
		%ytick={0.01, 0.02, 0.02, 0.03, 0.04, 0.05, 0.06},
		ylabel = {Bandwidth (B)},
		ylabel shift=-5pt,
		yticklabel shift={0cm},
		axis background/.style={fill=white},
		legend columns=1,
		legend style={legend cell align=left, align=left, fill=none, draw=none,inner sep=-0pt, row sep=0pt, font=\scriptsize},
		legend pos = north west,
		%
		%ymajorgrids,
		%xmajorgrids,
		%grid style={line width=.1pt, draw=gray!90,dashed},
		%major grid style={line width=.1pt,draw=gray!50},
		minor y tick num=5,
		%legend style={at={(.97,0.76)}},
		]
		% \addplot [color=A, solid, mark=diamond*, mark options={solid, A}]
		% table[row sep=crcr]{%
		% 	1 11.0790\\ % 11.0790 ms
		% 	2 21.0162\\  %21.0162 ms
		% 	3 30.7832\\ 
		% 	4 40.9725\\ 
		% 	5 50.7883\\
		% };
		% \addlegendentry{E-seaML}

        \addplot [color=E, solid, mark=asterisk, mark options={solid, E}]
		table[row sep=crcr]{%
                1 19899 \\ 
			2 39699 \\ 
			3 59499 \\ 
			4 79299 \\ 
			5 99099 \\ 
		};
		\addlegendentry{\nano~(SH)}

  
		\addplot [color=A, solid, mark=diamond*, mark options={solid, A}]
		table[row sep=crcr]{%
			1 46530\\ % 
			2 92730\\ % 
			3 138930\\ % 
			4 185130\\ % 
			5 231330\\ %
		};
		\addlegendentry{\nano~(MS)}
		
		\addplot [color=B, dashed, mark=square*, mark options={solid, B}]
		table[row sep=crcr]{%
			1 40185826.7\\ % 
			2 171803374.528\\ % 
			3 377695613.042\\ % 
			4 688368653.819\\ % 
			5 1058070416.142\\ % 
		};
		\addlegendentry{MicroFedML$_1$}

		\addplot [color=C, loosely dotted, mark=triangle*, mark options={solid, C}]
		table[row sep=crcr]{%
			1 49711211.023\\ % 
			2 101139782.452\\ % 
			3 150663591.976\\ % 
			4 202092163.404\\ % 
			5 251615972.928\\ % 
		};
		\addlegendentry{MicroFedML$_2$(50)}


		\addplot [color=H, dashed, mark=pentagon*, mark options={solid, H}]
		table[row sep=crcr]{%
			1 9376320\\ % 
			2 11027520\\ %
			3 12678720\\ %
			4 14329920\\ %
			5 15981120\\ % 
		};
		\addlegendentry{\FlamingoServerFirst}

		\addplot [color=D, loosely dotted, mark=otimes*, mark options={solid, D}]
		table[row sep=crcr]{%
			1 38552576\\ %
			2 41854976\\ %
			3 45157376\\ %
			4 48459776\\ %
			5 51762176\\ % 
		};
		\addlegendentry{\FlamingoServerSec}


	\end{axis}


\end{tikzpicture}%

